Graph-based Logic and Sketches

We present the basic ideas of forms (a generalization of Ehresmann's sketches) and their theories and models, more explicitly than in previous expositions. Forms provide the ability to specify mathematical structures and data types in any appropriate category, including many types of structures (e.g. function spaces) that cannot be specified by sketches. We also outline a new kind of formal logic (based on graphs instead of strings of symbols) that gives an intrinsically categorial definition of assertion and proof for each type of form. This formal logic is new to this monograph. The relationship between multisorted equational logic and finite product theories is worked out in detail.

==> ARTHEAD.tex <==
\typeout{This is ARTHEAD.tex 22 October 1996}

\makeatletter




\message{sections and parts,}
\renewcommand\thesubsubsection{\thesubsection\@alph\c@subsubsection}


\message{new symbols,}

\long\def\put(#1,#2)#3{\@killglue\raise#2\unitlength\hbox to \z@{\kern
#1\unitlength #3\hss}\message{.}\ignorespaces}

%% \def\thebibliography#1{\section*{References\@mkboth
%%  {REFERENCES}{REFERENCES}}\list
%%   {[\arabic{enumi}]}{\settowidth\labelwidth{[#1]}\leftmargin\labelwidth
%%   \advance\leftmargin\labelsep
%%   \usecounter{enumi}}
%%   \def\newblock{\hskip .11em plus .33em minus .07em}
%%   \sloppy\clubpenalty4000\widowpenalty4000
%% \sfcode`\.=1000\relax}
%%  \let\endthebibliography=\endlist

\def\doubleslash{//\penalty\exhyphenpenalty}
\def\pd{.}


\mathchardef\gt="313E %relation
\mathchardef\lt="313C %relation
\mathchardef\lte="0214 %\leq, with class of ordinary char
\mathcode`<="4268 %left delimiter
\mathcode`>="5269 %right delimiter
\mathcode`:="203A
\mathchardef\bq="4060
\mathchardef\eq="5027
\mathchardef\lsb="005B %left square bracket
\mathchardef\rsb="005D
%\def\ap{\kern 1pt\raise 1.4ex \hbox{$\mathchar"37A$}\kern 1pt}
\def\[{[\kern-1.2pt [}
\def\]{]\kern-1.2pt ]}
\def\R{{\bbold R}}
\def\Z{{\bbold Z}}
\def\Q{{\bbold Q}}
\def\N{{\bbold N}}
\def\o{\mathrel{\raise.3ex\hbox{$\scriptscriptstyle\circ$}}}





\message{changes in parameters,}

\lefthyphenmin=3 \setcounter{secnumdepth}{3}
\setcounter{tocdepth}{1}

\def\MakeUppercase#1{#1}

\message{constructed symbols,}
\def\epi{\mathrel{\mathchar"221\mkern -12mu\mathchar"221}}
\def\leftepi{\mathrel{\mathchar"220\mkern -12mu\mathchar"220}}
\def\mon{\mathrel{\m@th\hbox to 14.6pt{\lasy\char'51\kern-2pt$\arrext$\hss
$\mathord\rightarrow$}}} % width of \epi
\def\leftmono{\mathrel{\m@th\hbox to
14.6pt{$\mathord\leftarrow$\hss$\arrext$\kern-2pt\lasy\char'50%
}}} % width of \epi

\mathchardef\arrext="0200       % amr minus for arrow extension (see \into)
\def\addtotextheight#1{\advance\textheight by #1 \advance\@colht by #1
   \advance\@colroom by @1 \advance\vsize by #1}
\def\relstack#1#2#3{\mathrel{\mathop{#1}\limits^{%
    \textstyle#2}\limits_{\textstyle#3}}}
% \def\pf{\par\addvspace{\medskipamount}\noindent Proof.\emskip}
\def\Box{\vbox{\hrule\hbox{\vrule\kern.5ex
   \vbox{\kern1ex}\kern.5ex\vrule}\hrule}}
\newcommand\epf{~\hfill$\Box$\par\addvspace{\medskipamount}}

\newmuskip\tinymuskip
\tinymuskip=1.3mu
\renewcommand{\o}%
{\raise.2ex\hbox{$\scriptstyle\mskip\tinymuskip\circ\mskip\tinymuskip$}}

\newcommand{\op}{^{\rm op}}

\message{renamed symbols,}

\newcommand{\ba}{\mapsto}
% \newcommand{\e}{\exists}
\newcommand{\imp}{\Rightarrow}
\newcommand{\x}{\times}
\renewcommand{\a}{\forall}
\newcommand{\divides}{\mathbin{|}}

\message{command builders,}

%% SOME OF THESE ARE REPEATED IN LGHD1022
\def\mathopdef#1{\expandafter\def\csname#1\endcsname{%
\mathop{\mbox{\rm #1}}\nolimits}}
\def\logopn#1{\expandafter\def\csname#1\endcsname{%
{\mathop{\mbox{\sf #1}}\nolimits}}}
\def\logord#1{\expandafter\def\csname#1\endcsname{%
{\mathord{\mbox{\sfi #1}}}}}
\def\mathopdef#1{\expandafter\def\csname#1\endcsname{{\mathop{#1\,}}}}
\def\mathbfdef#1{\expandafter\def\csname#1\endcsname{{\hbox{\rm\bf #1}}}}
\def\mathrmdef#1{\expandafter\def\csname#1\endcsname{{\hbox{\rm #1}}}}
\def\mathttdef#1{\expandafter\def\csname#1\endcsname{{\hbox{\tt #1}}}}
%% \def\mathcatname#1{\expandafter\def\csname#1\endcsname%
%% {\mbox{\catname #1}}}
\def\mathsketchname#1{\expandafter\def\csname#1\endcsname%
{\mbox{\sketchname #1}}}
\def\mathskd#1{\expandafter\def\csname#1\endcsname%
{\mbox{\skd #1}}}
\def\mathcatname#1{\expandafter\def\csname#1\endcsname{%
\mathop{\catname{#1\fake}}\nolimits}}


\message{new environments,}

% \input bezier.sty


% ENVIRONMENTS

\itemsep\smallskipamount\parsep0pt\topsep\medskipamount
\newcounter{lister}
\newcounter{underlister}

\newenvironment{reflist}{\vskip 4ex plus 1ex minus .2ex {\large\bf
\noindent References} \begin{trivlist}}{\end{trivlist}}

\newenvironment{romanlist}
{\begin{list}{(\roman{lister})}%
{\usecounter{lister}}}%begin text
{\end{list}}% end text
\newcommand{\romlist}{\begin{romanlist}}
\newcommand{\eromlist}{\end{romanlist}\noindent}

\newenvironment{alphalist}
{\begin{list}{\alph{lister})}%
{\usecounter{lister}}}%begin text
{\end{list}}% end text
\newcommand{\alist}{\begin{alphalist}}
\newcommand{\ealist}{\end{alphalist}\noindent}

\newenvironment{squishlist}
{\begin{list}{\alph{lister})}%
{\usecounter{lister}\parsep0pt\itemsep 0pt plus 2pt}}%begin text
{\end{list}}% end text
\newcommand{\sqlist}{\begin{squishlist}}
\newcommand{\esqlist}{\end{squishlist}\noindent}

\newenvironment{labeledlist}[1]
{\begin{list}{{#1.\arabic{lister}}}{\usecounter{lister}
\settowidth{\labelwidth}{#1.9}\leftmargin\labelwidth\advance\leftmargin
by \labelsep\parsep0pt\itemsep 0pt plus 2pt}}
{\end{list}}%



\newenvironment{underlist}[1]
{\begin{list}{{\rm#1--\arabic{underlister}}}{\usecounter{underlister}
\parsep0pt\settowidth{\labelwidth}{#1--1}
\leftmargin\labelwidth \advance\leftmargin by \labelsep
}}%begin text
{\end{list}}%



\message{new commands,}

\def\umlaut{\"}

\mathrmdef{dom}
\mathrmdef{cod}
\mathrmdef{id}
\mathrmdef{source}
\mathrmdef{target}
\mathrmdef{Hom}
\mathrmdef{ev}
\mathrmdef{Lim}
\mathrmdef{lim}
\mathrmdef{colim}

\def\darray{\begingroup\arraycolsep 2em
     \def\arraystretch{1.5}\array}
\def\enddarray{\endarray\endgroup}

% \def\a#1{\Asc_{#1}}
% \def\N#1{\mbox{\skd #1}}

\newcommand{\thm}{\specialsubsection{Theorem}\begingroup\em}
\newcommand{\thl}{\specialsubsection{Lemma}\begingroup\em}
\newcommand{\thp}{\specialsubsection{Proposition}\begingroup\em}
\newcommand{\thcv}{\specialsubsection{Convention}\begingroup\em}
\newcommand{\thc}{\specialsubsection{Corollary}\begingroup\em}
\newcommand{\defn}{\specialsubsection{Definition}\begingroup\rm}
\newcommand{\notat}{\specialsubsection{Notation}\begingroup\rm}
\newcommand{\rem}{\specialsubsection{Remark}\begingroup\rm}
\newcommand{\rems}{\specialsubsection{Remarks}\begingroup\rm}
\let\defd=\defn
\newcommand{\exam}{\specialsubsection{Example}\begingroup\rm}
\newcommand{\fp}{\specialsubsection{Fine points}\begingroup\rm}
\newcommand{\warning}{\specialsubsection{Warning}\begingroup\rm}
\newcommand{\meth}{\specialsubsection{Method}\begingroup\rm}
\newcommand{\spec}{\specialsubsection{Specification}\begingroup\rm}
\newcommand{\ethm}{\endgroup\par\pagebreak[2]\addvspace{\medskipamount}}
\let\eth=\ethm
\let\ethc=\ethm
\let\ethcv=\ethm
\let\ethp=\ethm
\let\eexam=\ethm
\let\ethl=\ethm
\let\edefn=\ethm
\let\enotat=\ethm
\let\erem=\ethm
\let\erems=\ethm
\let\emeth=\ethm
\let\espec=\ethm
\let\ewarn=\ethm
\let\efp=\ethm
\def\pf{\specialsubsection*{Proof}}

\renewcommand{\sb}[2]{\{#1 \;\mid\;{#2}\}} % \sb was subscript

\def\bfdef{\bf}

\def\beqa{\begin{equation}\begin{array}{c}}
\def\eeqa{\end{array}\end{equation}\vskip 1ex\noindent}
% \def\itm{\item\hskip-1em}
\newcommand{\bc}{\begin{center}}
\def\beq{\begin{equation}}%for numbered equations and
\newcommand{\blist}[1]{\begin{labeledlist}{#1}}
\newcommand{\bp}{\begin{picture}}
\newcommand{\btable}{\begin{center}\begin{tabular}}
\newcommand{\ec}{\end{center}}
\def\eeq{\end{equation}}
\newcommand{\elist}{\end{labeledlist}}
\newcommand{\ep}{\end{picture}}
\newcommand{\etable}{\end{tabular}\end{center}}
%



%SPECIAL CHARACTERS

\def\|{\mathord{\mid}}

%\newcommand{\divides}{\mathbin{|}}
%\newcommand{\op}{^{\rm op}}
%\newcommand{\x}{\times}
%\renewcommand{\o}{\circ}%originally danish letter
%\newcommand{\ab}{\relax}
%\newcommand{\ov}{{\rm over}}
%\newcommand{\wrsym}{\mathop{\rm wr}\nolimits}
%\renewcommand{\wr}{\wrsym^}
%\renewcommand{\|}{\,\mid\,}

\newcommand{\0}{\emptyset}
\newcommand{\Cap}{\bigcap}
\newcommand{\Cup}{\bigcup}
\newcommand{\Deltop}{\mathbin{\Delta}}
\newcommand{\FALSE}{\mbox{\scriptsize FALSE}}
\newcommand{\Meet}{\bigwedge}
\newcommand{\Or}{\vee}%don't use "or" -- it's used in case
\newcommand{\Orrel}{\mathrel{\vee}}
\newcommand{\Orord}{\mathord{\vee}}
\newcommand{\Orbin}{\mathbin{\vee}}
\newcommand{\Rel}{\mathop{\rm Rel}\nolimits}
\newcommand{\Rplus}{\R^{\mathord{+}}}
\newcommand{\SQRT}{\mathop{\scriptsize SQRT}\nolimits}
\newcommand{\SQ}{\mathop{\scriptsize SQUARE}\nolimits}
\newcommand{\TRUE}{\mbox{\scriptsize TRUE}}
\newcommand{\ab}[1]{\left|#1\right|}
\newcommand{\alpharel}{\mathrel{\mbox{$\alpha$}}}
\newcommand{\alt}[2]{(\forall #1\mathord:#2)}
\newcommand{\al}[1]{(\forall #1)}
\newcommand{\all}{\forall}
\newcommand{\bra}{\{\}}
\newcommand{\ch}{\divides}%for choice in production
\newcommand{\cls}{\mbox{\rm cls}}
\newcommand{\comp}{^c}
\newcommand{\dash}{---}
\newcommand{\dollar}{\$}  %$
\newcommand{\e}{\mathop{\rm e}\nolimits}
\newcommand{\ext}[2]{(\exists #1\mathord:#2)}
\newcommand{\ex}[1]{(\exists #1)}
\newcommand{\fs}[2]{\mbox{$\lsb#1\!\rightarrow\!#2\rsb$}}%function space
\newcommand{\gka}{\alpha}
\newcommand{\gkb}{\beta}
\newcommand{\gks}{\sigma}
\newcommand{\gkt}{\tau}
\newcommand{\gkg}{\gamma}
\newcommand{\gte}{\geq}
\newcommand{\gtbin}{\mathbin{\gt}}
\newcommand{\geqbin}{\mathbin{\geq}}
% \newcommand{\id}{\mathop{\rm id}\nolimits}
\def\implies{\Rightarrow}
\newcommand{\impliesord}{\mathord{\Rightarrow}}
\newcommand{\impliesbin}{\mathbin{\Rightarrow}}
\newcommand{\inord}{\mathord{\in}}
\newcommand{\inbin}{\mathbin{\in}}
\newcommand{\includedin}{\subseteq}
\newcommand{\inc}{\subseteq}
\newcommand{\intersect}{\cap}
\newcommand{\inverse}{^{-1}}
\newcommand{\iso}{\cong}
\newcommand{\join}{\vee}
\newcommand{\lab}{\left|}
\newcommand{\lsq}{\mbox{`}}%use in math mode to get single quote
\newcommand{\ltbin}{\mathbin{\lt}}
\newcommand{\leqbin}{\mathbin{\leq}}

\newcommand{\meet}{\wedge}
\newcommand{\mt}{\wedge}
\newcommand{\nn}{\hspace{-.5em}}
\newcommand{\n}{\mbox{\bf n}}
\newcommand{\pa}{\vfill\newpage}
\newcommand{\pws}{\Psc}
\newcommand{\rab}{\right|}
\newcommand{\res}{\divides}%for restriction
\newcommand{\rsq}{\mbox{'}}
\newcommand{\st}[1]{`#1\rsq}
\newcommand{\tl}{\leftarrow}
% \newcommand{\toleft}{\gets}
\newcommand{\uext}[2]{(\exists!\,#1\mathord:#2)}
\newcommand{\uex}[1]{(\exists!\,#1)}
\newcommand{\union}{\cup}
\newcommand{\us}{\Usc}%universal set
\newcommand{\uu}{\underline}
\newcommand{\yields}{\mbox{\large\ $\vdash$ }}
% \newcommand{\yields}{\mbox{\large$\vdash$}}

\renewcommand{\.}{\cdot}
\renewcommand{\Join}{\bigvee}%originally bowtie symbol
\renewcommand{\and}{\wedge}%Latex uses it for titles
\newcommand{\andord}{\mathord{\wedge}}
\newcommand{\andbin}{\mathbin{\wedge}}
\newcommand{\andrel}{\mathrel{\wedge}}
\renewcommand{\a}{\mbox{\bf a}}
\renewcommand{\equiv}{\Leftrightarrow}
\newcommand{\equivord}{\mathord{\Leftrightarrow}}
\newcommand{\equivbin}{\mathbin{\Leftrightarrow}}
\renewcommand{\i}{\cap}
\renewcommand{\lq}{``}
\renewcommand{\pmod}[1]{\allowbreak \mkern8mu ({\rm mod}\,\,#1)}
\renewcommand{\rq}{''}
\renewcommand{\u}{\cup}


\newcommand{\strinc}%
  {\mathrel{\mathop{\subset}%
  \hspace{-.75em}{\raisebox{-.75ex}{$\scriptstyle\neq$}}}}
\let\oldclude=\subset

\def\twodots{\mathinner{\ldotp\ldotp}}

\newcommand{\lst}[3]{#1_{#2},\ldots,#1_{#3}}
\newcommand{\lstsb}[3]{(#1_i\mid i\in #2\twodots #3)}

% \newcommand{\bfi}[1]{\index{#1}{\large\bf #1}}
% \newcommand{\bfi}[1]{\index{#1}{\bf #1}}
% \def\text#1{\:{\rm #1}\:}

\newcommand{\rinf}[2]{#1\;\yields\; #2}
\newcommand{\einf}[2]{\rinf{#1}{#2}\;\mbox{and}\;\rinf{#2}{#1}}
\newcommand{\fracl}[2]{\frac{\,#1\,}{#2}}
\newcommand{\sepp}{\hspace{1 em}}%
\newcommand{\law}[2]{$$#1\eqno{\mbox{#2}}$$}

% \newcommand{\cod}{\mathop{\rm cod}\nolimits}
% \newcommand{\dom}{\mathop{\rm dom}\nolimits}

\def\pbox(#1,#2)#3{\put(#1,#2){\mbox{#3}}}
%\def\putbox(#1,#2)#3{\put(#1,#2){\makebox(0,0){#3}}}
\def\relstack#1#2#3{\mathrel{\mathop{#1}\limits^{#2}\limits_{#3}}}
\newcount \repetitions
\def\repto#1{
\repetitions=0
\loop\ifnum\repetitions<#1
    \advance \repetitions by 1
    \relbar\joinrel
\repeat
\rightarrow
}
\def\reptwo#1{\vcenter{\hbox{\ooalign{\raise3pt \hbox{$\repto{#1}$}
\crcr \lower2pt\hbox{$\repto{#1}$}}}}}
\def\TO{\relbar\joinrel\relbar\joinrel\relbar\joinrel\rightarrow}
\def\TWOO{\vcenter{\hbox{\ooalign{\raise3pt \hbox{$\TO$}\crcr
    \lower2pt\hbox{$\TO$}}}}}
\def\TWO{\mathrel{\mathpalette\TWOO{}}}
\def\Tofro{\mathrel{\mathpalette\Toofro{}}}
\def\Toofro{\vcenter{\hbox{\ooalign{\raise3pt \hbox{$\longrightarrow$}
     \crcr \lower2pt\hbox{$\longleftarrow$}}}}}
\def\To{\longrightarrow}
\def\Twoo{\vcenter{\hbox{\ooalign{\raise3pt \hbox{$\longrightarrow$}
     \crcr \lower2pt\hbox{$\longrightarrow$}}}}}


\mathcatname{Set}
\mathcatname{Cat}
\mathcatname{Gr}
\mathcatname{Th}
\mathcatname{Mod}





\def\emph#1{{\em#1\/}}
\def\MAX{\mathbin{\rm max}}
\def\MIN{\mathbin{\rm min}}
\def\MOD{\mathbin{\rm mod}}
\def\DIV{\mathbin{\rm div}}
\def\TRUNC{\mathop{\rm trunc}\nolimits}
\def\FLOOR{\mathop{\rm floor}\nolimits}
\def\cons{\mathop{\rm cons}\nolimits}
\def\head{\mathop{\rm head}\nolimits}
\def\tail{\mathop{\rm tail}\nolimits}
\def\source{\mathop{\rm source}\nolimits}
\def\target{\mathop{\rm target}\nolimits}
\def\GCD{\mathop{\rm GCD}\nolimits}
\def\LCM{\mathop{\rm LCM}\nolimits}
\def\ABS{\mathop{\rm ABS}\nolimits}
\def\Im{\mathop{\rm Im}\nolimits}


%% The following makes small-print ragged-right marginal notes
% \def\@parboxrestore{\@arrayparboxrestore%
% \let\\=\@normalcr\raggedright}
\long\def\@savemarbox#1#2{\global\setbox#1\vtop{\hsize\marginparwidth
   \@parboxrestore\raggedright\footnotesize #2}}
\long\def\mpar#1{{\marginpar{{#1}}}}

%% \def\mpar#1{{%
%% \def\@parboxrestore{\@arrayparboxrestore\let\\=\@normalcr\raggedright}
%% \marginpar{{\footnotesize #1}}}}

\def\darray{\begingroup\arraycolsep 2em
     \def\arraystretch{1.5}\array}
\def\enddarray{\endarray\endgroup}



\message{Bibliography commands,}

\makeatletter
\let\@internalcite\cite
\def\cite{\def\citeauthoryear##1##2{##1, ##2}\@internalcite}
\def\shortcite{\def\citeauthoryear##1##2{##2}\@internalcite}
\def\@biblabel#1{\def\citeauthoryear##1##2{##1, ##2}[#1]\hfill}



\long\def \@gobble #1{}
\long\def \@gobbletwo #1#2{}
\long\def \@gobblefour #1#2#3#4{}
\long\def\@firstofone#1{#1}
\long\def\@firstoftwo#1#2{#1}
\long\def\@secondoftwo#1#2{#2}
\def\@citex[#1]#2{%
  \let\@citea\@empty
  \@cite{\@for\@citeb:=#2\do
    {\@citea\def\@citea{,\penalty\@m\ }%
     \edef\@citeb{\expandafter\@firstofone\@citeb}%
     \if@filesw\immediate\write\@auxout{\string\citation{\@citeb}}\fi
     \@ifundefined{b@\@citeb}{\mbox{\bf ?}%
       \typeout{Citation `\@citeb' on page \thepage \space undefined}}%
       {\csname b@\@citeb\endcsname}}}{#1}}



\makeatother


% The following are for use when you don't use BibTeX.
% \def\book#1#2#3{{{\mbox{#1}}, }%
%    {{\bf #2. }}{#3.}\pagebreak[3]}
% \def\art#1#2#3{{{\mbox{#1}}, }%
%    {{\it #2. }}{#3.}\pagebreak[3]}
% \def\artc#1#2#3#4#5#6{{{\mbox{#1}}, }%
%    {{\it #2. }}{#3} {{\bf #4}} (#5), #6.\pagebreak[3]}
%
% \def\lnm#1{Lec\-ture Notes in Math\-e\-ma\-tics {\bf#1}}
% \def\lncs#1{Lec\-ture Notes in Com\-pu\-ter Sci\-ence {\bf#1}}
% \def\springer{Sprin\-ger-Ver\-lag }
% \def\cahiers#1{Cah\-iers de Topo\-lo\-gie et G\'e\-o\-m\'e\-trie
% Dif\-f\'e\-ren\-ti\-elle\ifnum#1>25 { Cat\-\'e\-go\-rique}\fi\ {\bf #1}}

\def\Frac#1#2{\frac{\displaystyle #1}{\displaystyle #2}}
\def\Rule#1#2{\Frac{\hspace{1em}#1\hspace{1em}}{#2}}
\makeatother

\makeatletter
\def\dmparms{
\normalsize
\@lowpenalty 151
\@medpenalty 651
\@highpenalty 1051
\@beginparpenalty -\@lowpenalty
\@endparpenalty -\@lowpenalty
\@itempenalty -\@lowpenalty
\binoppenalty=5000
\relpenalty=300
\clubpenalty=300
\widowpenalty=1000
\hyphenpenalty=15
\hfuzz=1pt
\emergencystretch=10pt
\thinmuskip=2.2mu
\medmuskip = 3.5mu plus 0.2mu minus .75mu
\thickmuskip = 5mu plus 3mu
%% \oddsidemargin 0.5in \evensidemargin 0.5in
%%  \topmargin 0pt \headheight 12pt \headsep 25pt \footskip 30pt
%% \textheight = 7.8in
%% \advance\textheight by \topskip
%% \textwidth 5.5in % changed from 5 in
\columnsep 10pt \columnseprule 0pt
\parskip 0pt plus 1.5pt
\parindent 1.5em
%% \topsep 10pt plus 4pt minus 6pt
%% \partopsep 3pt plus 2pt minus 2pt
\itemsep 5pt plus 2.5pt minus 1pt
\onecolumn}\makeatother

\message{setting values of counters}
\newcommand{\setpart}[1]{\setcounter{part}{#1}}
\newcommand{\setchap}[1]{\setcounter{chapter}{#1}}
\newcommand{\setsec}[1]{\setcounter{section}{#1}}
\newcommand{\setsubsec}[1]{\setcounter{subsection}{#1}}
\newcommand{\setpage}[1]{\setcounter{page}{#1}}
\typeout{End of arthead.tex}

